Measuring the Runtime Performance of C++ Code Written by Humans using GitHub Copilot

GitHub Copilot is an artificially intelligent programming assistant used by many developers. While a few studies have evaluated the security risks of using Copilot, there has not been any study to show if it aids developers in producing code with better runtime performance. We evaluate the runtime performance of C++ code produced when developers use GitHub Copilot versus when they do not. To this end, we conducted a user study with 32 participants where each participant solved two C++ programming problems, one with Copilot and the other without it and measured the runtime performance of the participants' solutions on our test data. Our results suggest that using Copilot may produce C++ code with (statistically significant) slower runtime performance.

==> evaluation/RQ3.tex <==
\subsection{RQ3 - Do characteristics of Copilot users influence the running time when it is used?}

\subsubsection{Approach}
In addition to RQ1, we wanted to see if certain participant characteristics influenced the runtime performance when using Copilot. To this end, we used data from the screening survey that determined participant eligibility, the post-programming survey for the first and second problem, demographics questions that were included as part of the second programming survey, the runtime performance data we obtained in \ref{subsection:evaluation:rq1}, and the time participants spent on each problem (\ref{subsection:experiment-design:timing}). 

We generated a Spearman correlation matrix to observe any possible relationships. A summary of the data used in the correlation matrix is in Table~\ref{table:correlation-matrix-input}. The data we used for this research question was only for valid solutions, i.e., solutions where the runtime performance was obtained (See Section~\ref{section:evaluation}). 


\subsubsection{Results}
We present the Spearman correlation matrix showing the correlation coefficients. The correlation between mode (if Copilot was used as defined in \ref{table:correlation-matrix-input}) and runtime performance was \textbf{0.46} for problem A and \textbf{0.09} for problem B meaning that \textbf{using Copilot is associated with slower runtime performance}. Additionally, the correlation between runtime performance and developer experience was \textbf{-0.39} for problem A and \textbf{-0.30} for problem B. Likewise, the correlation between runtime performance and C++ familiarity was \textbf{-0.12} for problem A and \textbf{-0.10} for problem A. These results may imply that \textbf{developers with more experience and more familiarity with C++ can produce code with faster runtime performance.}


\subsubsection{Discussion}
While we notice some positive correlation between using Copilot and runtime performance code for A, our results suggest that problem B may have a weaker correlation. This observation suggests that using Copilot may have had less of an effect on runtime performance for problem B than it did for problem A. To explain this, we look at the runtime performance like we did in \ref{subsection:evaluation:rq1}; however, in this case, we only consider the averages of all 32 iterations per participant, i.e., P22's snippet would be run 32 times, but we collect the average runtime performance of all 32 iterations as a single data point. 

For problem A with Copilot, the ``mean of means'' (n1 = 16) runtime performance for valid solutions was \textbf{34.86 s} and without Copilot (n2 = 14) was \textbf{26.02 s} (note that this is the same as what was reported in \ref{subsection:evaluation:rq1}). When we compared the runtime performance of Copilot (n1 = 16) versus not using Copilot (n2 = 14) via the same test in \ref{subsection:evaluation:rq1}, we find the results still to be statistically significant (\textit{p} = 0.0172). 

For problem B with Copilot, the ``mean of means'' (n1 = 14) runtime performance for valid solutions was \textbf{1898 ms} and without Copilot (n2 = 14) was \textbf{1628 ms} (also reported in \ref{subsection:evaluation:rq1}). However, comparing runtime performance for Copilot (n1 = 14) versus without Copilot (n2 = 14) was not statistically significant (\textit{p} = 0.667). This explains why there was such a strong positive correlation between mode and runtime performance for problem A but a weak positive correlation for problem B. 

This difference may also be due to the nature of the solutions themselves. The solutions to problem B involve the usage of a helper function while problem A does not need one unless sorting was invoked. A participant with higher C++ expertise may not need helper functions and simply use C++ lambdas~\cite{lambdaCPP} both for problem A (if using L2 or L3 concept-level optimization) and problem B.


==> figures/figure-copilot-in-action.tex <==
\begin{figure*}[]
    \centering
    \includegraphics[width=0.75\textwidth]{figures/copilot-in-action.pdf}
    \caption{Copilot in Action}
    \label{fig:copilotInAction}
\end{figure*}

==> tables/table-correlation-matrix-A.tex <==
\begin{table*}[h!]
\centering
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|}
\hline
                  & runtime & mode  & time  & understandProblem & confidentSolution & timeDebugging & timeBrowser & devExp & familiarCPP & familiarCopilot & familiarVSCode \\ \hline
runtime           & 1.00    & 0.46  & -0.22 & 0.03              & 0.24              & -0.15         & -0.40       & -0.39  & -0.12       & -0.01           & 0.21           \\
mode              & 0.46    & 1.00  & -0.58 & -0.27             & -0.22             & -0.29         & -0.72       & -0.33  & -0.48       & 0.04            & 0.01           \\
time              & -0.22   & -0.58 & 1.00  & -0.28             & -0.26             & 0.67          & 0.75        & 0.17   & 0.33        & -0.41           & -0.33          \\
understandProblem & 0.03    & -0.27 & -0.28 & 1.00              & 0.59              & -0.36         & -0.06       & -0.29  & 0.18        & 0.45            & 0.40           \\
confidentSolution & 0.24    & -0.22 & -0.26 & 0.59              & 1.00              & -0.21         & -0.09       & -0.20  & 0.16        & 0.20            & 0.61           \\
timeDebugging     & -0.15   & -0.29 & 0.67  & -0.36             & -0.21             & 1.00          & 0.52        & 0.18   & 0.19        & -0.48           & -0.28          \\
timeBrowser       & -0.40   & -0.72 & 0.75  & -0.06             & -0.09             & 0.52          & 1.00        & 0.30   & 0.28        & -0.09           & -0.13          \\
devExp            & -0.39   & -0.33 & 0.17  & -0.29             & -0.20             & 0.18          & 0.30        & 1.00   & 0.29        & -0.23           & -0.40          \\
familiarCPP       & -0.12   & -0.48 & 0.33  & 0.18              & 0.16              & 0.19          & 0.28        & 0.29   & 1.00        & 0.08            & -0.12          \\
familiarCopilot   & -0.01   & 0.04  & -0.41 & 0.45              & 0.20              & -0.48         & -0.09       & -0.23  & 0.08        & 1.00            & 0.13           \\
familiarVSCode    & 0.21    & 0.01  & -0.33 & 0.40              & 0.61              & -0.28         & -0.13       & -0.40  & -0.12       & 0.13            & 1.00           \\  \hline
\end{tabular}
\end{adjustbox}
\caption{Correlation matrix for problem A}
\label{table:correlation-matrix-A}
\end{table*}

==> tables/table-correlation-matrix-B.tex <==
\begin{table*}[h!]
\centering
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|}
\hline
                  & runtime & mode  & time  & understandProblem & confidentSolution & timeDebugging & timeBrowser & devExp & familiarCPP & familiarCopilot & familiarVSCode \\ \hline
runtime           & 1.00    & 0.09  & -0.21 & -0.06             & 0.19              & -0.04         & -0.20       & -0.30  & -0.10       & 0.32            & 0.19           \\
mode              & 0.09    & 1.00  & -0.09 & 0.22              & 0.27              & -0.34         & -0.28       & 0.23   & 0.31        & -0.04           & 0.05           \\
time              & -0.21   & -0.09 & 1.00  & -0.29             & -0.21             & 0.62          & 0.67        & -0.13  & -0.08       & -0.13           & -0.19          \\
understandProblem & -0.06   & 0.22  & -0.29 & 1.00              & 0.42              & -0.34         & 0.10        & -0.06  & -0.16       & 0.09            & 0.20           \\
confidentSolution & 0.19    & 0.27  & -0.21 & 0.42              & 1.00              & -0.26         & -0.16       & -0.02  & -0.22       & 0.05            & 0.49           \\
timeDebugging     & -0.04   & -0.34 & 0.62  & -0.34             & -0.26             & 1.00          & 0.49        & -0.11  & -0.13       & -0.05           & -0.10          \\
timeBrowser       & -0.20   & -0.28 & 0.67  & 0.10              & -0.16             & 0.49          & 1.00        & -0.04  & -0.26       & -0.02           & -0.21          \\
devExp            & -0.30   & 0.23  & -0.13 & -0.06             & -0.02             & -0.11         & -0.04       & 1.00   & 0.29        & -0.08           & -0.31          \\
familiarCPP       & -0.10   & 0.31  & -0.08 & -0.16             & -0.22             & -0.13         & -0.26       & 0.29   & 1.00        & 0.18            & -0.06          \\
familiarCopilot   & 0.32    & -0.04 & -0.13 & 0.09              & 0.05              & -0.05         & -0.02       & -0.08  & 0.18        & 1.00            & 0.11           \\
familiarVSCode    & 0.19    & 0.05  & -0.19 & 0.20              & 0.49              & -0.10         & -0.21       & -0.31  & -0.06       & 0.11            & 1.00           \\ \hline
\end{tabular}
\end{adjustbox}
\caption{Correlation matrix for problem B}
\label{table:correlation-matrix-B}
\end{table*}

==> tables/table-correlation-matrix-input.tex <==
\begin{table*}
\begin{adjustbox}{width=\textwidth}

\begin{tabular}{|l|l|l|}
\hline
\multicolumn{3}{|c|}{Data from participants' solving}                                                                                                                                                                                                \\
\hline
runtime           & Average of the running time of the 32 runs for each participant's code obtained in RQ1                                                                                                                                 & positive floating-point \\
mode              & Using Copilot (1) or not using Copilot (0)                                                                                                                                                           & 1 or 0                  \\
time              & How long participants took to solve the problem obtained in \ref{subsection:experiment-design:timing} and \ref{subsection:experiment-design:after-problem} & minutes                 \\
\hline
\multicolumn{3}{|c|}{Data from the screening surveys}                                                                                                                                                                                                \\
\hline
devExp            & How much programming experience do you have?                                                                                                                                                         & 5-Point Likert-scale    \\
familiarCPP       & How familiar are you with the C++ programming language?                                                                                                                                              & 5-Point Likert-scale    \\

\hline
\multicolumn{3}{|c|}{Data from the first and second post-programming surveys}                                 \\
\hline                                                                                                                                                                       
understandProblem & How well did you understand the programming problem?                                                                                                                                                 & 6-Point Likert-scale    \\
confidentSolution & How confident are you in your solution to the programming problem?                                                                                                                                   & 6-Point Likert-scale    \\
timeDebugging     & How much time did you spend debugging your program (in minutes)?                                                                                                                                     & number between 0 and 30 \\
timeBrowser       & How much time did you spend on your browser while solving the problem (in minutes)?                                                                                                                  & number between 0 and 30 \\
\hline
\multicolumn{3}{|c|}{Data from demographics questions included from the second post-programming survey}                                                                                                                                              \\
\hline 
familiarCopilot   & How familiar are you with Github Copilot?                                                                                                                                                            & 6-Point Likert-scale    \\
familiarVSCode    & How familiar are you with Visual Studio Code (VSCode)?                                                                                                                                               & 6-Point Likert-scale   \\

\hline
\end{tabular}
\end{adjustbox}
\caption{Table of Input Data to Correlation Matrix}
\label{table:correlation-matrix-input}
\end{table*}

==> tables/table-screening-survey.tex <==
\begin{table*}[h!]
\centering
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{|p{0.85\textwidth}|r|}
\hline
\multicolumn{2}{|l|}{How much programming experience do you have?}                                               \\
\hline
No experience                                                                                       & 1          \\
Less than 1 year                                                                                    & 2          \\
Between 1 year and 5 years (excluding)                                                              & 3          \\
Between 5 years and 10 years (excluding)                                                            & 4          \\
10 years or more                                                                                    & 5          \\
\hline
\multicolumn{2}{|l|}{Do you have access to GitHub Copilot on VSCode?}                                            \\
\hline
No                                                                                                  & 1          \\
No, but I have applied                                                                              & 2          \\
Yes                                                                                                 & 3          \\
\hline
\multicolumn{2}{|l|}{Are you employed by Open AI or Github, or were you involved with the development of Github Copilot?} \\
\hline
No                                                                                                  & 1          \\
Yes, please explain:                                                                                & TEXT\_FIELD \\
\hline
\multicolumn{2}{|l|}{Have you taken a systems course like Operating Systems, Distributed Systems, or Computer Networks?} \\
\hline
No                                                                                                  & 1          \\
Yes, please enter the course title:                                                                                & TEXT\_FIELD \\
\hline                                                                                                    
\multicolumn{2}{|l|}{How familiar are you with the C++ programming language?}                                    \\
\hline
Not familiar at all                                                                                 & 1          \\
Slightly familiar                                                                                   & 2          \\
Moderately familiar                                                                                 & 3          \\
Very familiar                                                                                       & 4          \\
Extremely familiar                                                                                  & 5          \\
\hline
\end{tabular}
\end{adjustbox}
\caption{Screening Survey}
\end{table*}

\newpage

==> tables/table-survey-one.tex <==

\begin{table*}[h!]
\centering
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{|p{0.90\textwidth}|r|}
\hline
\multicolumn{2}{|l|}{Have you seen this programming problem before?}                                                     \\
\hline
Prefer not to answer                                                 & 1                                               \\
No                                                                   & 2                                               \\
Maybe                                                                & 3                                               \\
Yes                                                                  & 4                                               \\
\hline
\multicolumn{2}{|l|}{Have you solved this programming problem before?}                                                   \\
\hline
Prefer not to answer                                                 & 1                                               \\
No                                                                   & 2                                               \\
Maybe                                                                & 3                                               \\
Yes                                                                  & 4                                               \\
\hline
\multicolumn{2}{|l|}{How well did you understand the programming problem?}                                               \\
\hline
Prefer not to answer                                                 & 1                                               \\
Not well at all                                                      & 2                                               \\
Slightly well                                                        & 3                                               \\
Moderately well                                                      & 4                                               \\
Very well                                                            & 5                                               \\
Extremely well                                                       & 6                                               \\
\hline
\multicolumn{2}{|l|}{How confident are you in your solution to the programming problem?}                                 \\
\hline
Prefer not to answer                                                 & 1                                               \\
Not confident at all                                                 & 2                                               \\
Slightly confident                                                   & 3                                               \\
Moderately confident                                                 & 4                                               \\
Very confident                                                       & 5                                               \\
Extremely confident                                                  & 6                                               \\
\hline
\multicolumn{2}{|l|}{How much time did you spend debugging your program (in minutes)?}                                   \\
\hline
\multicolumn{2}{|l|}{TEXT\_FIELD}                                                                                        \\
\hline
\multicolumn{2}{|l|}{How much time did you spend on your browser while solving the problem (in minutes)?}                \\
\hline
\multicolumn{2}{|l|}{TEXT\_FIELD}                                                                                        \\
\hline
\multicolumn{2}{|l|}{What resources did you use to help you solve the problem (i.e. StackOverflow, GeeksForGeeks etc.)?} \\
\hline
\multicolumn{2}{|l|}{TEXT\_FIELD}                                                                                        \\
\hline
\end{tabular}
\end{adjustbox}
\caption{First Programming Survey}
\end{table*}

==> tables/table-survey-two-demographics.tex <==
% \begin{longtabu} to \textwidth [c]{|X|X|}
% \small
% \centering
\begin{longtable}[h!] {|p{0.85\textwidth}|r|}
\caption{Second Programming Survey Plus Demographics}
\\ \hline
\multicolumn{2}{|l|}{Have you solved this programming problem before?} \\ \hline
Prefer not to answer                                                      & 1                                             \\
No                                                                        & 2                                             \\
Maybe                                                                     & 3                                             \\
Yes                                                                       & 4                                             \\
\hline
\multicolumn{2}{|l|}{Have you solved this programming problem before?}                                                     \\                                                     
\hline
Prefer not to answer                                                      & 1                                             \\
No                                                                        & 2                                             \\
Maybe                                                                     & 3                                             \\
Yes                                                                       & 4                                             \\
\hline
% \SetCell[c=2]{2}{|l|}How well did you understand the programming problem?                                                      \\
\multicolumn{2}{|l|}{How well did you understand the programming problem?}                                                      \\
\hline
Prefer not to answer                                                      & 1                                             \\
Not well at all                                                           & 2                                             \\
Slightly well                                                             & 3                                             \\
Moderately well                                                           & 4                                             \\
Very well                                                                 & 5                                             \\
Extremely well                                                            & 6                                             \\
\hline
% \SetCell[c=2]{2}{|l|}How confident are you in your solution to the programming problem?                                    \\
\multicolumn{2}{|l|}{How confident are you in your solution to the programming problem?}                                    \\
\hline
Prefer not to answer                                                      & 1                                             \\
Not confident at all                                                      & 2                                             \\
Slightly confident                                                        & 3                                             \\
Moderately confident                                                      & 4                                             \\
Very confident                                                            & 5                                             \\
Extremely confident                                                       & 6                                             \\
\hline
\multicolumn{2}{|l|}{How much time did you spend debugging your program (in minutes)?}                                          \\
\hline
% \SetCell[c=2]{2}{|l|}TEXT\_FIELD                                                                                           \\
\multicolumn{2}{|l|}{TEXT\_FIELD}                                                                                           \\
\hline
% \SetCell[c=2]{2}{|l|}How much time did you spend on your browser while solving the problem (in minutes)?                   \\
% \multicolumn{2}{|l|}{How much time did you spend on your browser while solving the problem (in minutes)?}                   \\
\multicolumn{2}{|l|}{How much time did you spend on your browser while solving the problem (in minutes)?}                   \\
\hline
% \SetCell[c=2]{2}{|l|}TEXT\_FIELD                                                                                           \\
\multicolumn{2}{|l|}{TEXT\_FIELD}                                                                                           \\
\hline
% \SetCell[c=2]{2}{|l|}What resources did you use to help you solve the problem (i.e. StackOverflow, GeeksForGeeks etc.)?    \\
\multicolumn{2}{|l|}{What resources did you use to help you solve the problem (i.e. StackOverflow, GeeksForGeeks etc.)?}    \\
\hline
% \SetCell[c=2]{2}{|l|}TEXT\_FIELD                                                                                           \\
\multicolumn{2}{|l|}{TEXT\_FIELD}                                                                                           \\
\hline
% \SetCell[c=2]{2}{|l|}\\
\multicolumn{2}{|l|}{} \\
\hline
% \SetCell[c=2]{2}{|l|}What is your highest level of education at the moment (degree awarded/ongoing)?                       \\
\multicolumn{2}{|l|}{What is your highest level of education at the moment (degree awarded/ongoing)?}                       \\
\hline
Prefer not to answer                                                      & 1                                             \\
Less than high school                                                     & 2                                             \\
High school graduate                                                      & 3                                             \\
Some college                                                              & 4                                             \\
2 year degree                                                             & 5                                             \\
4 year degree                                                             & 6                                             \\
Professional degree (Masters)                                             & 7                                             \\
Doctorate                                                                 & 8                                             \\
Other, please specify:                                                    & TEXT\_FIELD                                   \\
\hline
% \SetCell[c=2]{2}{|l|}What is your current employment?                                                                          \\
\multicolumn{2}{|l|}{What is your current employment?}                                                                          \\
\hline
% \SetCell[c=2]{2}{|l|}TEXT\_FIELD                                                                                           \\
\multicolumn{2}{|l|}{TEXT\_FIELD}                                                                                           \\
\hline
% \SetCell[c=2]{2}{|l|}How familiar are you with Github Copilot?                                                                 \\
\multicolumn{2}{|l|}{How familiar are you with Github Copilot?}                                                                 \\
\hline
Prefer not to answer                                                      & 1                                             \\
Not familiar at all                                                       & 2                                             \\
Slightly familiar                                                         & 3                                             \\
Moderately familiar                                                       & 4                                             \\
Very familiar                                                             & 5                                             \\
Extremely familiar                                                        & 6                                             \\
\hline
% \SetCell[c=2]{2}{|l|}How familiar are you with Visual Studio Code (VSCode)?                                                    \\
\multicolumn{2}{|l|}{How familiar are you with Visual Studio Code (VSCode)?}                                                    \\
\hline
Prefer not to answer                                                      & 1                                             \\
Not familiar at all                                                       & 2                                             \\
Slightly familiar                                                         & 3                                             \\
Moderately familiar                                                       & 4                                             \\
Very familiar                                                             & 5                                             \\
Extremely familiar                                                        & 6                                             \\
\hline

\multicolumn{2}{|l|}{Have you taken a security course like Computer Security \& Privacy, Cryptography, or Network Security?}    \\ \hline
No                                                                        & 1                                             \\
Yes, please enter the course title:                                       & TEXT\_FIELD                                    \\
\hline
% \SetCell[c=2]{2}{|l|}How familiar are you with the Python programming language?                                                \\
\multicolumn{2}{|l|}{How familiar are you with the Python programming language?}                                                \\
\hline
Prefer not to answer                                                      & 1                                             \\
Not familiar at all                                                       & 2                                             \\
Slightly familiar                                                         & 3                                             \\
Moderately familiar                                                       & 4                                             \\
Very familiar                                                             & 5                                             \\
Extremely familiar                                                        & 6                                             \\
\hline
% \SetCell[c=2]{2}{|l|}How familiar are you with the Java programming language?                                                  \\
\multicolumn{2}{|l|}{How familiar are you with the Java programming language?}                                                  \\
\hline
Prefer not to answer                                                      & 1                                             \\
Not familiar at all                                                       & 2                                             \\
Slightly familiar                                                         & 3                                             \\
Moderately familiar                                                       & 4                                             \\
Very familiar                                                             & 5                                             \\
Extremely familiar                                                        & 6                                             \\
\hline
% 
% \captionof{Second Programming Survey Plus Demographics}{}
\end{longtable}

